End User Authoring of Personalized Content Classifiers: Comparing Example Labeling, Rule Writing, and LLM Prompting

Existing tools for laypeople to create personal classifiers often assume a motivated user working uninterrupted in a single, lengthy session. However, users tend to engage with social media casually, with many short sessions on an ongoing, daily basis. To make creating personal classifiers for content curation easier for such users, tools should support rapid initialization and iterative refinement. In this work, we compare three strategies -- (1) example labeling, (2) rule writing, and (3) large language model (LLM) prompting -- for end users to build personal content classifiers. From an experiment with 37 non-programmers tasked with creating personalized moderation filters, we found that participants preferred different initializing strategies in different contexts, despite LLM prompting's better performance. However, all strategies faced challenges with iterative refinement. To overcome challenges in iterating on their prompts, participants even adopted hybrid approaches such as providing examples as in-context examples or writing rule-like prompts.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> sections/12_old_related_work.tex <==
\section{Related Work}
\subsection{Personalized Content Curation Tools for End-Users}
% content curation is an important thing for internet users, and they want to have more personalization. Personal content moderation more specifically means ....
% What do end-users need for content curation tools? they are easily distracted, want to entertain and relax, do not care the most about curation performance, their preferences are nuanced and subtle. Content curation tools for end-users should take these user needs into considerations.

% There are three strategies commonly used in literature to support end-user to customize an algorithm. There are a body of tools developed around each strategy.
% But they failed to consider much user needs in the context of content curation. 

% what are content curation tools specifically designed for end-users? 
% They also have some shortcomings, for instance, require technical understanding (regular expressions), too little customization space.


Despite the indispensable role online communities play in our daily lives, we still see with disappointment an overwhelming amount of spam, misinformation, and off-topic posting in our online experiences~\cite{PervasiveHarrassment}. Major social media platforms like Facebook ~\cite{FacebookAlgorithm}, YouTube ~\cite{YoutubeAlgorithm}, and Reddit ~\cite{Chandrasekharan2019} have deployed algorithms to remove inappropriate content at scale automatically. However, such centralized platform-wide moderation might fail to account for cultural variances across countries~\cite{jiang2021understanding}, communities~\cite{weld2022makes}, or diverse individual preferences, potentially leading to unintended harms. 
Consequently, there are increasing calls for personal content moderation~\cite{jhaver2023personalizing, jhaver2023users, he2023cura, burrell2019users, konstan2012recommender}.

We define personal content moderation as \textit{a form of moderation in which users can customize some aspects of their moderation preferences based on the content of posts submitted by other users}~\cite{jhaver2023personalizing, jhaver2023users}. Critics and scholars anticipate that users can have greater control and transparency in moderation as the content moderation decision-making moves from centralized platforms towards individual users~\cite{engler2022middleware, masnick2019protocols}. In particular, there are two kinds of personal moderation scenarios. The first involves end-users removing unwanted content from their personalized content feeds on platforms like Instagram, TikTok, and Twitter~\cite{jhaver2023personalizing}. The second scenario occurs when individuals moderate for a small community, such as the comment section of YouTube videos or Discord servers~\cite{jhaver2022designing}. Compared to large online communities with dedicated teams of moderators, these individuals must manage their moderation roles with limited time and resources.

Within this trend, online platforms have started to experiment and offer personal content moderation tools, which can be divided into two categories: \textit{account-based} and \textit{content-based}. Account-based moderation tools enable users to mute or block an account to prohibit future interaction with it. For instance, Blockbots in Twitter supports the curation of a shared blocklist of accounts~\cite{jhaver2018online, geiger2016bot}. In comparison, content-based moderation tools help users configure their preferences based on the content alone. The Most popular tool is \textit{word filters}~\cite{jhaver2022designing} which allow users to configure a list of block words. Any content that includes block words will then be removed or held for manual inspection. Some online platforms have also enabled users to adjust their sensitivity for some common concepts, such as racism, misogyny, and political views~\cite{Instagram2024, bhargava2019gobo, Bodyguard2024}. In this work, we focused specifically on content-based personal moderation tools rather than account-based ones. While various platforms maintain different types of account-related information such as reputation~\cite{movshovitz2013analysis} and the number of followers, content-based tools focus directly on the content itself, making them more universally applicable across different platforms and scenarios.

There are two critical stages when end-users create their personal moderation filters: \textbf{communicating preferences} and \textbf{iterating filters}. Initially, users must articulate their personal preferences in a format that moderation filters can understand, such as compiling a list of relevant keywords for a word filter. Subsequently, the iteration stage involves identifying and correcting errors in the filter. This cycle does not conclude with the filter's initial configuration but continues over the long term, as end-users might identify mistakes in their everyday use of personal moderation filters~\cite{shen2021everyday}. Sometimes, they might only realize their moderation needs upon encountering certain content~\cite{jhaver2023personalizing}. 
% While we recognize that these two stages are often intertwined in the interactive creation process~\cite{fails2003interactive}, these two stages are supported by different functionalities of a personal moderation system and therefore deserve separate examination. 

In particular, explainability is closely associated with iterability. Prior research has shown that a deeper understanding of how an algorithm functions enables end-users to more effectively debug a filter's faults~\cite{ko2008debugging, fiebrink2011human}. In the absence of explainability, users might experience difficulty building accurate mental models of the algorithm, potentially leading to misinformed user behavior~\cite{kulesza2012tell, tullio2007works}. 
However, explanations also present additional information and risk overloading users~\cite{ghai2021explainable}. 
For explanations to effectively support end-users in training their binary algorithms, they must be actionable. This means that they should not only expose the misalignment between algorithms and users but also offer pathways to refine and improve their algorithms~\cite{kulesza2015principles}.



\subsection{Interactive Machine Learning for Text Classification}
Despite the ubiquitous use of machine learning algorithms in a wide variety of domains, only a small group of people with technical expertise possess the skills to develop these algorithms. In contrast, interactive machine learning (IML) democratizes the training of ML models, enabling non-experts to participate through "rapid, focused, and incremental model updates"~\cite{amershi2014power}. 
% This approach has been successfully implemented in various fields, from classifying legal and medical documents ~\cite{wallace2012deploying, vsavelka2015applying}, to image search by concept ~\cite{fogarty2008cueflik}, and fraud 
In this paper, we view personal moderation tools as a kind of interactive machine learning system for text classification.
The interactive machine learning process encompasses three critical phases:(1) Users begin by examining the model's outputs across a set of examples; (2) They then offer feedback to the model, guiding its learning in the desired direction; (3) Lastly, users assess the model's overall performance and decide whether to conclude the training process~\cite{amershi2011designing, stumpf2009interacting}. At the heart of this process lies the \textit{teaching vocabulary}--the framework through which users structure their feedback ~\cite{porter2013interactive}. 
There is a variety of teaching vocabularies, ranging from assigning labels to selecting features, specifying parameters, and indicating error preferences~\cite{kapoor2010interactive}. In the following, we review the two most commonly used teaching vocabularies—\textit{labels} and \textit{features}—and highlight their current relationships to content moderation tools.

First, many IML systems often consider end-users as oracles that provide correct labels. In particular, techniques like pretrained word-embeddings~\cite{devlin2018bert} and active learning~\cite{settles2009active} are often used to minimize the number of labels required to effectively train a machine learning algorithm~\cite{settles2009active}. An active learner iteratively picks examples for labeling from an unlabeled dataset through query sampling strategies, such as uncertainty sampling~\cite{lewis1995sequential} and query-by-committee~\cite{seung1992query}. 
% In particular, the uncertainty sampling strategy samples instances the algorithm is the least certain about how to label~\cite{lewis1995sequential}. 
% For instance, a probabilistic model for binary classification would select instances whose posterior probability of being positive is nearest 0.5. 
Previous studies have shown that people find labeling effective for communicating with opaque, "black-box" algorithms~\cite{jhaver2023personalizing, feng2024mapping}.
However, researchers have criticized that end-users might find the repetitive task of labeling data tedious and not transparent~\cite{das2013end}. Furthermore, there is a risk that users might apply labels inconsistently due to evolving criteria~\cite{kulesza2014structured}.
Amidst these challenges, researchers are developing moderation algorithms using labels that are gathered from online communities~\cite{chandrasekharan2019crossmod, halfaker2020ores}, leveraging the fact that end-users who frequently interact with recommendation algorithms via implicit or explicit labels~\cite{zhao2013interactive, yi2014beyond, kang2022you} are already familiar with training algorithms in this way.

Responding to the aforementioned criticisms of the labeling approach, a growing body of research has begun to enable feature-level human input~\cite{hema2006active, wallace2012deploying, vsavelka2015applying}. Here, the term ``feature'' refers to an attribute of a data instance that
is useful for predicting the class label. In the context of text classification tasks, features often refer to the mentions or weights of keywords.
% Prior research has shown that people often have a good intuition for important features in text classification tasks.
Although the empirical results on whether feature-level input from end-users improves performance have been mixed~\cite{hema2006active, das2013end, wu2019local}, there is a general agreement that feature-level input is more
efficient (i.e., requires fewer user actions) to achieve comparable results to example labeling and that it could produce models more closely aligned with an individual's needs or domain knowledge. On the other hand, features can be seen as too granular and therefore not generalizable enough, posing a challenge for end-users in creating effective filters~\cite{Chandrasekharan2019, song2023modsandbox}.

How these features are exploited by algorithms varies. They can be directly incorporated into transparent machine learning algorithms such as Decision Tress, Naive Bayes algorithms~\cite{kulesza2015principles}, and Support Vector Machines~\cite{vsavelka2015applying}. For example, almost all social media platforms allow users to curate a list of blocked words to filter out undesirable content~\cite{jhaver2022designing}. As the most widely used content moderation tool in Reddit~\cite{song2023modsandbox, jhaver2019human, chandrasekharan2019crossmod}, AutoMod further enables community moderators to write regular expressions to remove posts that violate community guidelines~\cite{jhaver2019human}. 
In addition, as end-users might produce noisy and inconsistent features~\cite{das2013end, boecking2020interactive}, user-generated features can also be used to label the unlabeled data. 
Algorithms like weak supervision algorithms then learn from these ``soft labels''~\cite{ratner2017snorkel}. But these indirect approaches sacrifice the transparency and control that users often assume with feature-level input. For this reason, IML systems designed for end-users often integrate features with transparent ML algorithms to give users stronger mental models of algorithms~\cite{kulesza2015principles, vsavelka2015applying}.

% In this study, inspired by the interactive machine learning literature, we focus on two specific forms of personal moderation tools designed to allow end-users to encode their complex preferences into algorithms. 
% The first type allows end-users to label \textbf{examples} within an active learning framework. The second type enables users to specify a list of keywords \textbf{rules}. While it's common for many IML systems to accept user inputs in both labels and features~\cite{wallace2012deploying, vsavelka2015applying}, we intentionally separate these two forms of input to closely examine the end-users' abilities and perception regarding each type of input. Besides, we only consider the system where features are incorporated directly into transparent ML algorithms as we want to investigate how transparency influences the overall user experience and the effectiveness of the system.

\subsection{Large Language Models and In-Context Learning}
Large language models (LLMs) have exploded in popularity due to their proficiency in a broad spectrum of natural language processing tasks, such as sentiment analysis and machine translation. Rather than having to train a new model for every custom task, users can just customize the model by feeding it natural language \textbf{prompts} at run time. Such ability to recognize the desired task on-the-fly is called \textit{in-context learning}~\cite{brown2020language}. In particular, LLMs' application in content moderation has recently attracted substantial interest~\cite{franco2023analyzing, kumar2023watch, OpenAI2024GPT4}. They are expected to detect unwanted content effectively and therefore reduce the potential emotional burdens for human reviewers. Research has shown that, even without finetuning, LLMs can outperform state-of-art classifiers in detecting toxic content, especially achieving a better balance in the precision-recall trade-off~\cite{kumar2023watch}. However, LLMs face challenges in applying more complex and nuanced moderation policies that go beyond simple hate speech or toxicity filtering~\cite{kolla2024llm}. Sometimes they might even perform worse than a coin toss~\cite{kumar2023watch}. 

Developing effective natural language prompts for in-context learning is crucial to leveraging LLMs in content moderation~\cite{min2022rethinking, mishra2021cross}. To date, the most common patterns for prompting are either \textit{zero-shot} or \textit{few-shot} prompts. Zero-shot prompts simply give instructions for the task without any specific examples for training~\cite{wang2019survey}. Research indicates that the performance of zero-shot prompts can be enhanced through iterative refinement of task instructions~\cite{efrat2020turking} and by breaking down tasks into simpler components~\cite{wei2022chain}.
On the other hand, few-shot prompting incorporates a few input-output examples to showcase the desired pattern which LLMs should adhere to ~\cite{sahoo2024systematic, brown2020language}. The quality of few-shot prompts heavily relies on the example selections~\cite{rubin2021learning}. While few-shot prompts generally outperform zero-shot prompts, the simplicity of composing natural language instructions without the need for selecting examples makes zero-shot prompting an attractive option for end-users.

However, there are still challenges that hinder end-users from creating and refining their prompts. Research has shown that even a slight adjustment to the prompt format or the order of examples used can greatly influence the model performance ~\cite{sclar2023quantifying, lu2021fantastically}. In addition, due to individuals' varied perspectives, they often find it challenging to evaluate the clarity of their instructions and to align their perspectives with those of LLMs, leading to incorrect or unexpected answers~\cite{deng2023rephrase}. To help end-users identify effective prompts, researchers have proposed various tools that facilitate prompt design. For instance, many systems help users explore variants of prompt instructions and automatically compare their effectiveness~\cite{mishra2023promptaid, strobelt2022interactive}. Other efforts focus on helping users select the most relevant and representative examples for few-shot prompting~\cite{wu2023scattershot, levi2024intent}. 

% In this work, we consider \textbf{prompts} as another teaching vocabulary in addition to labels and features in the context of interactive machine learning. Users can provide natural language prompts to train an LLM to act as their personal moderator~\cite{ma2023adapting, OpenAI2024GPT4}. 
% In particular, we focus on employing LLMs for personal moderation rather than community or platform moderation in this work, as there are often more diverse user preferences but more limited resources for designing effective prompts. 
% Despite the growing interest in employing LLMs for content moderation, we would like to first examine whether designing prompts represents a more \textit{effective, efficient, and usable} way for personal moderation than labeling examples and configuring rules. 





==> sections/15_old_results.tex <==
\section{Results}
\begin{figure*}[ht!]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includesvg[width=\linewidth]{figures/accuracy.svg}
        \caption{\textbf{Accuracy}}
        \label{fig:accuracy}
    \end{subfigure}
    \medskip
    \begin{subfigure}{\textwidth}
        \centering
        \includesvg[width=\linewidth]{figures/precision.svg}
        \caption{\textbf{Precision}}
        \label{fig:precision}
    \end{subfigure}
    \medskip
    \begin{subfigure}{\textwidth}
        \centering
        \includesvg[width=\linewidth]{figures/f1.svg}
        \caption{\textbf{F1 Score}}
        \label{fig:f1score}
    \end{subfigure}
    \medskip
    \begin{subfigure}{\textwidth}
        \centering
        \includesvg[width=\linewidth]{figures/recall.svg}
        \caption{\textbf{Recall}}
        \label{fig:recall}
    \end{subfigure}
    \caption{\textbf{Comparison of Performance Metrics Over Time Across Three Experimental Systems}. This series of subfigures tracks the performance of filters created by participants, with updates every thirty seconds. Each subfigure represents one of the following metrics: accuracy, precision, recall, and F1 score. Together, they illustrate how the average values of these metrics evolved from the first minute to the end of the study across all participants. The value at the time 15:30 represents the final performance of the corresponding system. }
    \label{performance}
\end{figure*}

\subsection{Performance and Speed of Personal Moderation Systems}

Figure \ref{performance} displays a comparison of filter performances across the three systems, with the final point of each line indicating the final performance. Table \ref{effective models} presents the pairwise differences among the three systems. We observed no significant differences in accuracy across the three personal moderation systems. However, the prompt writing system demonstrated significantly higher recall compared to the example labeling system (Est.Diff = 0.205, $p$  < 0.001) and the rule configuring system (Est.Diff = 0.232, $p$  < 0.001). As for precision, although the rule system showed significantly higher precision than the example labeling system  (Est.Diff = 0.097, $p$  < 0.05), it did not significantly differ from the prompt system in precision. Consequently, the prompt system also achieved a significantly higher $F_1$ score than the other two systems (Est.Diff compared to rules = 0.105, $p$  < 0.01; Est.Diff compared to examples = 0.141, $p$ < 0.001). 

In summary, the prompt system proved more effective at removing unwanted content compared to the other two systems, although it did not demonstrate higher precision in its removal predictions. For users who prioritize recall or overall performance, our results indicate that the prompt system is the most effective of the three. However, for users who value precision, the prompt system and the rule system show comparable effectiveness.


\begin{table}[ht]
\centering
\captionsetup[table]{skip=10pt}
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
& \multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{F1 Score}} \\

Pairwise Comparison & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. \\
\hline
Rules - Examples & -0.004 & 0.019 & 0.097* & 0.040 & -0.027 & 0.053 & 0.036 & 0.038 \\
Prompts - Examples & -0.003 & 0.019 & 0.074 & 0.040 & 0.205*** & 0.053 & 0.141*** & 0.038 \\
Prompts - Rules & 0.001 & 0.019 & -0.023 & 0.040 & 0.232*** & 0.053 & 0.105** & 0.038 \\
\bottomrule
\end{tabular}
\hfill\\
\hfill\\
\caption{\textbf{Post-hoc pairwise t-test results for the final performance}: pairwise differences in mean performance metrics of the final filter participants developed using three experiment systems. $p$ < 0.001***, $p$ < 0.01**, $p$ < 0.05*}
\label{effective models}
\end{table}


\subsection{Efficiency of Personal Moderation Systems}
Figure \ref{performance} depicts the changes in the performance of the three personal moderation systems throughout the experiment. Table \ref{effective models at 7.5} and Table \ref{effective models at 4} present the pairwise differences in filter performance at 7.5 minutes and 4 minutes respectively. Consistent with our findings on overall effectiveness, the prompt writing system consistently exhibited significantly higher recall and $F_1$ scores compared to the other systems. In additionBesides, both the rule system and the prompt system showed greater precision than the example labeling system at 4 minutes (Est.Diff = 0.136, $p$ < 0.05; Est.Diff = 0.134, $p$ < 0.05 respectively). The precision of these two systems were not significantly different from each other. Across the duration of the task, there were no significant differences in accuracy among the three systems. However, we observed that both the prompt and the rule system have a steadily increasing recall but a gradually decreasing precision. This suggests that it is easier for participants to catch more unwanted content than to increase the specificity of their filter. 

In summary, our experiments showed that the prompt system proved more efficient at removing unwanted content compared to the other two systems throughout the task, although it did not demonstrate higher precision in its removal predictions than the rule system. For users who prioritize recall or overall performance, our results indicate that the prompt system is the most efficient of the three. However, for users who value precision, both the prompt system and the rule system exhibited comparable efficiency in accurately predicting removals.

\begin{table}[ht]
\centering
\captionsetup[table]{skip=10pt}
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
& \multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{F1 Score}} \\

Pairwise Comparison & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. \\
\hline
Rules - Examples & -0.004 & 0.020 & 0.136* & 0.058 & -0.090 & 0.059 & -0.003 & 0.047 \\
Prompts - Examples & 0.025 & 0.020 & 0.134* & 0.058 & 0.146* & 0.059 & 0.138** & 0.047 \\
Prompts - Rules & 0.029 & 0.020 & -0.002 & 0.058 & 0.236*** & 0.059 & 0.141** & 0.047 \\
\bottomrule
\end{tabular}
\hfill\\
\hfill\\
\caption{\textbf{Post-hoc pairwise t-test results for the filter performance at 4 minutes}: pairwise differences in mean performance metrics of the final filter participants developed using three experiment systems. $p$ < 0.001***, $p$ < 0.01**, $p$ < 0.05*}
\label{effective models at 4}
\end{table}



\begin{table}[ht]
\centering
\captionsetup[table]{skip=10pt}
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
& \multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Precision}} & \multicolumn{2}{c|}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{F1 Score}} \\

Pairwise Comparison & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. \\
\hline
Rules - Examples & 0.001 & 0.020 & 0.097 & 0.055 & -0.068 & 0.056 & 0.017 & 0.042 \\
Prompts - Examples & 0.026 & 0.020 & 0.133* & 0.055 & 0.197*** & 0.056 & 0.168*** & 0.042 \\
Prompts - Rules & 0.025 & 0.020 & 0.035 & 0.055 & 0.264*** & 0.056 & 0.152*** & 0.042 \\
\bottomrule
\end{tabular}
\hfill\\
\hfill\\
\caption{\textbf{Post-hoc pairwise t-test results for the filter performance at 7.5 minutes}: pairwise differences in mean performance metrics of the final filter participants developed using three experiment systems. $p$ < 0.001***, $p$ < 0.01**, $p$ < 0.05*}
\label{effective models at 7.5}
\end{table}



% \subsection{Usability of Personal Moderation Systems}




\subsection{Usability: Communicate Personal Preferences to Moderation filters}


\begin{figure*}
    \centering
    \includesvg[width=\textwidth]{figures/usability.svg}
    \caption{\textbf{Comparison of Subjective Measures Across Three Experimental Systems}. Participants were asked to rate their experience in terms of task load and usability. This figure displays the comparison of their ratings across three experimental systems. }
    \hfill
    \label{usability}
\end{figure*}

% \begin{table}[ht]
% \centering
% \captionsetup[table]{skip=10pt}
% \begin{tabular}{l|cc|cc|cc|cc}
% \toprule
% & \multicolumn{2}{c|}{\textbf{Easy to use}} & \multicolumn{2}{c|}{\textbf{Mental Demand}} & \multicolumn{2}{c|}{\textbf{Work Hardness}} & \multicolumn{2}{c}{\textbf{Hurried}} \\

% Pairwise Comparison & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. \\
% \hline
% Rules - Examples & 0.082 & 0.241 & 0.499* & 0.255 & 0.444 & 0.237 & 0.166 & 0.203 \\
% Prompts - Examples & -0.091 & 0.239 & 0.394 & 0.253 & 0.091 & 0.235 & 0.182 & 0.200 \\
% Prompts - Rules & -0.173 & 0.241 & -0.105 & 0.255 & -0.353 & 0.237 & 0.016 & 0.203 \\
% \bottomrule
% \addlinespace
% \addlinespace
% \toprule
% & \multicolumn{2}{c|}{\textbf{Good Understanding}} & \multicolumn{2}{c|}{\textbf{Difficult to correct}} & \multicolumn{2}{c|}{\textbf{Frustrated}} & \multicolumn{2}{c}{\textbf{Meeting needs}} \\

% Pairwise Comparison & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. & Estimate & Std. Err. \\
% \hline
% Rules - Examples & 0.286 & 0.230 & 0.671* & 0.289 & 0.648* & 0.279 & 0.160 & 0.257 \\
% Prompts - Examples & 0.030 & 0.227 & 0.576* & 0.286 & 0.545* & 0.277 & 0.121 & 0.255 \\
% Prompts - Rules & -0.256 & 0.230 & -0.096 & 0.289 & -0.103 & 0.279 & -0.039 & 0.257 \\
% \bottomrule
% \end{tabular}

% \caption{\textbf{Post-hoc pairwise t-test results for the filter performance at 7.5 minutes}: pairwise differences in mean performance metrics of the final filter participants developed using three experiment systems. $p$ < 0.001***, $p$ < 0.01**, $p$ < 0.05*}
% \label{effective models at 7.5}
% \end{table}


When end-users start to create their filter, the first step is to communicate their personal preferences to moderation filters using the allowed teaching vocabulary. The creating experience is influenced not only by how well each filter learns from the teaching vocabulary but also by how easily users can translate their preferences into this vocabulary.
The latter is particularly important in this process, especially since people often start with only a vague idea of their preferences. Below, we detail our findings regarding the creation experience across the three systems.

\subsubsection{\textbf{Example Labeling System}}
On average, participants labeled 138 examples in 15 minutes. Most participants found the process of labeling examples to be straightforward, involving simple binary decisions about whether a comment should be removed. While they considered labeling individual examples easy, they acknowledged that the task becomes progressively more demanding as more labels are required to develop an effective filter.
However, perceptions of this creating experience varied significantly between two distinct groups of participants. 

% [labeling is tiring] P6: even though one comment might not take a lot of work, the cumulative number of comments does take a lot of work.

The first group of participants often found their preferences grounded in individual moderation decisions and therefore found labeling examples an effective way to communicate their preferences to algorithms. 
Participants recognized that their moderation decisions were influenced by the content of comments, as well as their intuitive feelings. P4 noticed that ``\textit{sometimes it might be the entire sentence that I don't want to see, or maybe it's just about a word. ... It could also be the feeling of the comment you don't feel right about it}''. 
Therefore, labeling examples allowed them to express these nuanced preferences directly to the algorithm, without the need to distill such nuances into succinct rules or prompts. They also showed higher trust in algorithms' capabilities to discern implicit patterns and infer their preferences. 
Even though they acknowledged the tedious nature of labeling enough examples to effectively train their filter, they believed this was still less mentally demanding and more efficient than trying to summarize their high-level criteria themselves.
As P2 explained, ``\textit{I would actually trust the algorithm finding trends more as me looking at everything and trying to build my own ... especially with my lack of experience and lack of time}''.  

% [nuances as a result of personal identities] as described by P3: \textit{I'm able to go through each one and personally make that decision as to whether or not I want to see that common. But [in the other two systems], I have to rely on algorithms that doesn't know me or my experiences or identities.}

% [oppose the interactivity / authentic] P1: But like if I were to use a filter, I would want it to be as useful as possible, and because of the limitations of the rules, and like ChatGPT made several mistakes. It's like I would prefer for it to be as concise as possible. So even though it would be tiring, it's like it's more beneficial for me to do it right the first time.

In contrast, the second group of participants, who had clear high-level moderation preferences in mind, found labeling examples inefficient and ineffective for expressing their preferences. 
P13 clearly expressed his frustration with the inability to explicitly state his preferences: ``\textit{There are too many decisions to make. Yeah, they're small decisions of yes or no. But usually, I don't have to keep creating 50 small decisions to indicate my personal preferences. .. Why am I going through hundreds of these when I just want to focus on saying my preferences?}''
In addition, the frustration increased when participants could not find sufficient relevant examples to indicate their preferences to the filter, as described by P10, ``\textit{I feel like I have this criterion [remove violence calls] in my head. But there is nowhere I can label these examples}''. Finally, there were concerns about whether algorithms would accurately learn high-level preferences from labels. As P13 worried, ``\textit{what if all the comments happened to have [the word] Texas, so the AI just picks up those all related to Texas}''.

% P5: it is. I guess that is a limitation of having what the example labeling interface create a filter based on what you're inputting. It's trying to look for a path that may not exist if you're just doing it based on, like your intuition, or how you feel about the comment.

\subsubsection{\textbf{Rule Configuring System}}
Participants created an average of 3 rules. Of these rules, 65\% contained only one ``include'' condition, 18\% had two ``include'' conditions, and 14\% combined one ``include'' with an exception condition. Each condition, on average, consisted of 12 phrases. Many participants consider configuring rules efficient yet mentally taxing. Rule creation is inherently an iterative process that requires participants to continuously review examples and identify relevant words for inclusion in the filter. This task was often perceived as more mentally demanding than simply labeling examples. As explained by P6, ``\textit{To come up with more words, I have to read all the sentences, and it becomes the same thing [as labeling examples]. But I have to find and then write down the triggering word. So the write down the words is the extra work [compared to labeling examples], right?}''


Some of our findings resonate with previous research on word filters \cite{jhaver2022designing, jhaver2023personalizing, song2023modsandbox}. For example, while some participants appreciated the control that rules provided, many expressed frustration over the limitations of keyword-based content removal, which often overlooks the broader context surrounding the keywords. Despite systems features that suggested synonyms and detected spelling variants, participants still often encountered unexpected misspellings or similar phrases, and therefore complained about the difficulty of curating a comprehensive list of phrases.

While most prior work focused on how moderators developed and used word filters in their moderation practices, our study explores the challenges end-users face in translating their nuanced preferences into effective rules. First, participants struggled to convert some vague user preferences into specific keywords. For instance, P10 compared two kinds of user preferences: ``\textit{It is easier to think about specific words for removing profane content, but then for violence, I didn't know what words specifically to say [for such content].}'' This challenge was further compounded by the fact that moderation preferences often encompass multiple concepts, necessitating the use of more complex rule structures. For instance, P11 tried to create a rule to ``\textit{remove personal attacks against an organization}''. Even though she managed to compile two lists of phrases--one for ``personal attacks'' and another for ``organizations''--she found that a conjunction of these two concepts did not accurately capture the intended relationship between them. 

However, not all user preferences are nuanced, and rules excel at filtering content related to specific preferences. For instance, rules can effectively remove content with any explicit language with a comprehensive list of words. Participants also mentioned the use of rules to hide content about particular events. As P1 explained, ``\textit{I would only use the rule system if there was a particular topic that was very distressing for me, like a bombing somewhere. If I were personally affected by that and didn't want to hear anything about that, I would just create a short list of relevant words. }''


\subsubsection{\textbf{Prompt Writing System}}
Participants created an average of 4 prompts. On average, each prompt consisted of 96 characters, 1.13 positive examples, and 0.57 negative examples. Many participants found the prompt writing system more effective for identifying relevant, or even implicit, comments compared to other systems. For instance, writing prompts enabled them to express concepts more efficiently. P6 explained this advantage, ``\textit{for rules, if there are 1,000 words I don't want to see, I have to list all 1,000 words, [whereas for ChatGPT], I only need to think of 10 words among those 1,000 words, and then ChatGPT itself understands that this guy does not want this kind of words.}''. They can now describe concepts that are hard to describe with keywords, such as irrational comments or privacy disclosure. Additionally, writing prompts simplifies the articulation of complex preferences, like avoiding content related to self-harm or violent incidents, which would otherwise require complex rule structures.

% P6: like, if it works properly, then I think it might even be the best method out of the 3 cause you don't have to like. You don't have to think about a lot of words. So if you say words like stupid, then the range gets bigger, right? There are so many words that could fit inside the range. So it's easy and like I would not mind doing that. 

% P13: It's easier to get ChatGPT [to determine if] it is the majority of it, or if it doesn't have, these very strong words in it. And it's easier to show it the discourse, and then let it learn from whether they're just having an argument but it's turned into hateful speech.

% P10: I think in the beginning it it's about the same to set all of them up. I feel like cause a lot of them you have to change to make it correct for all of the comments.
% But then I feel like for that one. It's more. Once you get a filter that you'd like, it would be more adaptive for the rest of your comments that you get, and the other 2 don't adapt. They just stay consistent. I guess, with the labeling one. It's closer.

However, participants also encountered several challenges in articulating their preferences in prompts. First, some participants found it difficult to summarize high-level prompts from their intuitive moderation decisions on specific examples. As new content continuously flooded their social media feeds, they lacked ``\textit{a holistic view about what were the alarming comments}'' (P2). P3 elaborated on her confusion: ``\textit{some of the comments would contain similar content, but not exactly the same, and so I feel like it was hard to come up with something that captured all of them}''. While labeling examples provided an opportunity to identify trends among comments, participants complained that writing prompts required them to prematurely categorize unwanted content into broad groups.

Second, even though participants managed to write down their prompts, they pointed out an inherent disconnect in how humans and LLMs perceive the same prompts. Several noted that LLMs might interpret language differently, potentially leading to misinterpretations. They observed that ``descriptions could be very subjective'' (P4) and asked ``\textit{what has [LLM] previously been trained on? For words they labeled as extreme, I might not think as extreme}'' (P13). Besides, they suggested that LLM might not fully understand their experiences and personalities from just short prompts, and therefore might fail to execute their preferences faithfully. 

% P2: It did but I also think they were also nuanced. And I think it is just like. I felt comfortable, putting the ones that were acceptable into the box. But then it almost made me feel like I had to put every single one in. and I think because I feel like they were all kind of different in their own way, or someone who wrote it wrote it very. I don't like like slightly, they wrote it in a way that I feel like not every algorithm could perceive it to be very harmful.

% P2: Are you thinking about how it's hard for the algorithm to process such nuances? Or is it difficult for you to come up with a high-level description to cover all these nuances?
% Angela Tu: I feel like I feel like it's kind of both, like in terms of, I felt like the algorithm found it difficult when I applied the filter, but while creating the filter itself too. I felt like it was hard to put everything in there, even though I think it could be a lack of trust in the algorithm, too. But I think that's my, that was my thought process at the moment.

In reflection of such an inherent disconnect, participants found that they need to dedicate extra effort to describing concepts beyond LLMs' existing knowledge. For example, LLMs lacked awareness of the context, such as the video or post to which comments were attached. P7 wanted to remove irrelevant comments and wished ``\textit{ChatGPT to be familiar with the content of the original post}''. Additionally, LLMs often struggled with identifying misinformation or conspiracy theories, especially those related to politics. W14 experienced this limitation: ``\textit{I wanted to remove this comment because it contains obvious disinformation about the city of Portland Oregon, but my filter did not understand my definition of obvious disinformation.}''

Similarly, many participants noticed that LLMs tend to interpret their preferences broadly and therefore have poor performance in distinguishing different degrees of a concept. For instance, P13 noticed that ``\textit{it has the problem of differentiating between just like minor attacks on someone's character [such as fools] and ones that are strong and can be perceived as harm.}''. Similarly, P8 struggled to teach LLMs to ``\textit{differentiate between threats and just using the word 'shoot' or 'kill'}''. While participants can easily instruct LLMs on what is clearly bad or good, aligning LLMs with their moderation decisions in borderline cases remains a challenge. 

Consequently, several participants even opted to avoid using high-level descriptions and instead write prompts that resembled rules, such as ``\textit{Remove texts that refer to people as stupid, dumb, idiots [a list of words]}''. However, many participants recognized that writing prompts is inevitably an iterative process where they need to continuously review LLM predictions and refine their prompts accordingly. P10 described this process in detail: ``\textit{In the beginning, I have an idea of what I do not want to see and then I would submit that. But [AI] wouldn't know what I was talking about, so I had to change my wording to match what AI would understand. }'' For some participants, this process nudged them to actively reflect on their personal preferences, but for others, it was mentally demanding. P2 expressed her feelings, ``\textit{it was almost more tiring to write prompts [than labeling examples], as you need to think about each one, but then apply it, and then see one little thing you could have fixed, and then reapply it}''.

% P10: then the last one I had was just violence, but that one was hard to quantify with the filters, cause I was basing it off of like this one [Need to allow parents of that child to drop the shooter in the wood-chipper and record his screams for posterity. That would be a justice, of a sort.] This one was hard to capture with all of the filters,

% P8: Nona David: like, have their pros and cons cause the more narrow you get. It's like you might get to this like, really hyper, specific thing, and kind of lost the big picture. But then, if you have just like these larger generalizations, you know you can't get down to the nitty, gritty, and identify truly like exactly what phrases you want to remove. So I guess it's, I guess, just a matter of like what you want to focus on, whether it's like effectiveness or like ease of setting up that filter. But for me, I would say I liked the more specific, narrow filters myself.

%P12: if I could figure out more like what it considers to be discrimination or a broad group of people, then I could probably work with that.

% [help brainstorm prompts]
% P5: Hmm! Sometimes for comments If you didn't know what to classify it as you couldn't type in a prompt to filter it out because you didn't know how to type. So maybe I wrote like having the option to type in a comment. And then maybe having the AI generate suggestions based on the content of that like. Oh, this seems like it contains this. Do you want this moderated I think that could be useful.

% P12: like think of so many laws for example. We have laws against killing people. But we have exceptions to self-defense. I feel it would be problematic if you didn't have exceptions to the general concept of self-defense. There's an implicit idea in the don't kill people rule. But like the self-defense cover. Hopefully, that's a good enough analogy.

% P13: Tom Finnegan: if it's borderline on one of those, how much is that like helpful? And I can always just turn it off if I'm willing to try and look more deeply like at something, or if I want to get an unfiltered response.


\subsection{Usability: Iterate the Filter When Encountering a Mistake}
We have documented how end-users convey their nuanced preferences to moderation filters. Now, we shift our focus to another critical aspect of the creation process: how end-users iterate on their filters upon encountering mistakes. While we recognize that these two aspects are often intertwined in the interactive creation process, the iteration phase primarily involves understanding the filter’s errors and refining the filter accordingly. Furthermore, we observed that iterating based on mistakes is a common practice in the use of personal moderation tools, as users frequently identify mistakes made by the deployed filters and periodically update their filters.

\subsubsection{Example Labeling System} 
We examined participants' explanations about one false positive and one false negative in the survey. Echoing prior research about how end-users develop folk theories to make sense of content moderation~\cite{mayworm2024content, moran2022folk} or curation algorithms~\cite{eslami2016first, devito2017algorithms}, most participants found that they only had at most a vague understanding of why their filters made incorrect predictions. For example, some participants were puzzled why certain comments were not removed, saying that ``\textit{I thought the explicit language would be enough to remove the comment
}'' (P8). 
Others believed the algorithms were only identifying superficial features from their labeled examples. As P3 noted, ``\textit{I chose to remove comments that alluded to the act of murdering. But this one seems more of a statement of fact than a graphic representation}''. 
In comparison to the initial communicating stage, participants found it easier to articulate specific preferences the filter should learn from a mistake. As a result, they envisioned using rules or prompts to explain these mistakes to the filter for iterative improvements, an approach echoed in recent studies~\cite{piorkowski2023aimee, daly2021user}. 
In the absence of such features in the current system, participants suggested they wanted to label more similar examples to these mistakes to better teach the filter. 
 
% P8: I don't know. Now that you say this, I feel like, maybe I think that the AI would be apt to like, identify those changes just because they can, you know, sort of consume all this data. You know. Remember, you know, certain decisions that you made on social media, or like certain content you consumed. And then how that compares, you know, to content, you consume, you know, either later or like a week later. So that's interesting. Yeah.

% P8: To be honest. I guess it would matter how frequently you engage in that sort of activity. but yeah, I don't know that I would say that the labeling examples would be as effective and identifying sort of like these substantial, I guess, substantial, or like more minute changes.

% P12: But if the algorithm, it's like, I detect a small change in this person's behavior. Let's suggest this type of video because they think they may like that.

\subsubsection{\textbf{Rule Configuring System}}
Thanks to the transparency of the rule configuring system, participants had a clearer understanding of why their rule filters made incorrect predictions than the other two systems. This transparency facilitated iterative improvements in some cases. For example, participants could easily add phrases to address comments that used unexpected spelling variants or similar phrases. However, they encountered significant challenges when trying to address more nuanced contexts. First, some comments might be undesirable even without using any triggering words. Even if participants could identify such keywords, they sometimes hesitated to add them as it could lead to more mistakes. For instance, P2 voiced a concern, ``\textit{someone could use a profanity or bad word, but it could be used in a less harmful way. If I just put that profanity in there they will right away get rid of all these comments}''. Finally, while participants attempted to create more complex rule structures (e.g., adding another ``include''/``exclude'' condition) to account for more nuances, they often found this process mentally taxing and overly specific. As P5 indicated, ``\textit{Should I add a condition that applies to this comment only? Just so I can appease my own ease of getting rid of this comment, but it doesn't necessarily apply to other comments. Is it necessarily beneficial in the long run?}''

\subsubsection{\textbf{Prompt Writing System}}
Similar to the example labeling system, participants found that they only had a vague understanding of why their filter made mistakes. Nevertheless, unlike with the example labeling system where participants could not pinpoint specific labels that led to the mistake, the prompt writing system allowed them to review and reflect on the problematic prompt, providing a direction for further iteration.
P2 noted this advantage: ``\textit{the prompt system was more transparent in the sense that it highlights specific guidelines you have set up. You could then change them, and see what they do}''. The challenge of iterating prompts based on a mistake significantly depends on both the participants' understanding of the mistake and the complexity of their preferences.

On the one hand, participants recognized that some mistakes were due to unclear communication of their preferences to LLMs. Often, these errors were relatively straightforward to correct. For instance, many participants intended to remove only personal hate speech directed at specific individuals but failed to specify this in their prompts. Consequently, the filter also removed comments containing general hate speech. On the other hand, when the mistake suggested more nuances in moderation preferences, participants found it challenging to refine their prompts effectively. For instance, P12 wanted to be open to bipartisan discussions and aimed to keep comments if ``\textit{that person had a non-deeply seated partisan bias with the potential to change}''. Similarly, Participant W8 noted a misinterpretation: ``\textit{This comment got removed for the promotion of inflicting harm on oneself or others, but it should not have been removed because it is being used hypothetically in a metaphor.
}'' These subtle nuances proved difficult for participants to incorporate in their prompts.

On the other hand, participants believed that stemmed from a misalignment in understanding concepts between humans and LLMs. Common disagreements involved whether certain phrases should be classified within specific concepts, such as labeling ``fool'' as offensive, ``hell'' as obscene, or `losers` as derogatory.  W3 noted this issue, ``\textit{The filter must have identified some of the terms used in this statement as derogatory or offensive. The filter and I probably disagreed about the extent to which these terms could be seen as offensive.
}'' In such cases, participants frequently adjusted their prompt descriptions in various ways to test and improve their alignment with LLMs. P13 described how he iterated his prompt: ``\textit{I don't want any like demeaning attacks on personal intelligence, but the word 'fool' is like a very low one. So instead of saying any [personal attacks], I probably should have said extreme attacks, or give it examples of what I meant by that}''.

However, participants sometimes faced confusion due to the idiosyncratic behaviors of LLMs, leaving them unsure of how to make further improvements. For instance, P3 was perplexed by why the prompt filter removed the comment ``\textit{Jessica is the best}'':``\textit{I'm honestly not sure why the filter removed this content. I wrote something about removing comments with harmful descriptions, so maybe it thought that this description was harmful in some way.}'' In rare instances, participants were surprised that the prompt filter did not remove the same comment as the few-shot example, as P1 expressed her frustration: ``\textit{With ChatGPT, I would directly copy and paste a comment that I didn't want, and it still wouldn't remove it.}''. Even though the resultant performance of their prompt filters is comparable to the other two systems, such unpredictable behaviors significantly undermined their confidence in using LLMs for personal moderation. 

When unsure how to improve their prompts after encountering a mistake, participants often resorted to adding the incorrectly classified comments directly into their prompts as few-shot examples. In this process, they are essentially labeling examples rather than writing prompts. Four out of thirty-seven participants even included more than five examples in their prompts. Since labeling individual examples is considered straightforward, participants also found this method convenient for iterating on their prompts. W6 remarked: ``\textit{I liked that I could copy and paste certain examples in ChatGPT. It made it easier to capture ideas that specific words do not allude to but are alluded to by unique comments}''. However, some participants also recognized the limitations of this approach. As P13 noted, ``\textit{I think [adding examples to prompts] is good up to a certain extent. If you know there are comments you don't want, it's great and ... also gives you more nuances. But sometimes when a lot of these comments are extremely similar, [the ChatGPT] just gets confused}''.

% [transparency they want]
% P9: Yeah, I'd like to know what specific item triggered the prompt or with specific words or phrases. Yeah.


% P12:  There were some things where I was like “Hold on it. Just remove that like that is a broad generalization to a group of people Why, the heck did that include that? That should have been removed.

% P12: maybe if I could figure out more like what it considers to be discrimination or a broad group of people, then I could probably work with that.


\subsection{Factors Influencing Preferences of Personal Moderation Systems}

We asked participants to rank the three experiment systems regarding their preferences for using each in real-life personal moderation, as well as to explain their rationale for these rankings. 
Figure \ref{preferences} illustrates the distribution of participants' rankings. 
The Wilcoxon Signed-Rank test showed no significant differences between any of the three systems. 
Despite the growing enthusiasm for using LLMs for content moderation, we were surprised to find that a comparable number of participants still preferred labeling examples or configuring rules to create their personalized moderation filters.
Upon closely examining data from semi-structured interviews and open-ended responses in the final survey, we identified several dimensions that contribute to these diverse preferences. 
These dimensions underscore the principal differences across the three systems. Furthermore, a participant’s positioning on each dimension not only illustrates individual differences but also highlights the variety of personal moderation scenarios they encounter.

\begin{figure*}
    \centering
    \includesvg[width=0.7\textwidth]{figures/preferences.svg}
    \caption{\textbf{Distribution of Participant Preferences for Personal Moderation Systems}. This figure illustrates how participants ranked three systems as ``High'', ``Middle'' and ``Low'' in terms of preference for real-life personal moderation. Results from the Wilcoxon Signed-Rank test indicate no significant differences between any pair of systems.}
    \hfill
    \label{preferences}
\end{figure*}

\textbf{Whether people value explicit articulation of their preferences.} As discussed earlier, articulating personal preferences in high-level constructs like rules or prompts could be challenging sometimes. While some participants began creating filters with well-defined moderation preferences, others needed to review examples to form their own preferences. For them, example labels are a by-product of their review process and do not take extra effort. In addition, we observed that many participants often slightly changed their criteria after reviewing more examples, and more so in the long run. Sometimes these changes might be too subtle to notice. As a result, explicitly stated preferences can become outdated, whereas algorithms could potentially detect and adapt to these subtle changes in preferences. As P12 explained in detail, ``\textit{Preferences change over time, and we may not explicitly realize that. So you may accidentally remove some things if your preferences change but you have already explicitly set them in stone. Then you don't end up getting the new exposure}''. On the other hand, some participants appreciated the chance to actively reflect on and articulate their preferences through high-level constructs, despite the extra effort required.

% [the need to learn from examples] Angela Tu: But then I feel like with the label one. I've started seeing trends myself and so it made it easier to adjust my criteria accordingly.

\textbf{Whether people need to review more examples.} In our study, participants required fewer examples to develop an effective filter using the prompt writing system compared to the other systems. On average, participants reviewed 133 and 127 examples for the example filter and rule filter systems respectively, whereas only 53 examples were needed for the prompt filter system. The need to review numerous toxic examples can be distressing, particularly for those creating filters to block such content. P8 suggested the difference between moderation scenarios: ``\textit{if I were moderating for my own sake and not for a community, I would probably just focus more on the ease of creating a filter so that I don't have to subject myself to these potentially offensive comments.}'' In addition, there might not be many toxic examples available when people develop a filter for a new space. As P5 commented, ``\textit{if you were creating a channel afresh, you don't have those examples readily available to you}''.

\textbf{The trade-off between precision and recall.} Our participants demonstrated varied approaches to balancing precision and recall. Some were open to encountering controversial or toxic content and were cautious about falsely removing comments. P12 described his rationale as follows: ``\textit{My preference is to limit the number [of comments] that accidentally gets removed. I don't want to fall into any echo chamber. Even if there are really crazy people saying really crazy things, they make me frustrated, but I still should know about it}''.  Conversely, other participants preferred to avoid toxic content on their social media feeds and were less concerned about mistakenly removing benign content. P13 expressed his preference: ``\textit{Personally, too specific is worse than the too broad. If the filter keeps certain content I really don't want to see, that's far worse than if I didn't get an extra post. Because of how much content there already is, I'll just get others on my feed anyway.}'' For these users, the high recall of the prompt filter is even advantageous during the creation stage. Since LLMs could collect the most relevant, potentially unwanted examples with initial prompts, participants could focus on reviewing these examples to increase the precision of their prompts.
% P13: Tom Finnegan: I think if like, you're a moderator for someone else, you'll usually just err on the side of too broad because  I don't want negative comments getting to them. It is not really my content. And so I only want the non-borderline ones to be the first ones to show up. Just so that if anyone's going on there, they're less likely to feel triggered.

\textbf{Controllability and transparency.} An important distinction between the rule configuring system and the other two systems is its transparency. 
As P10 described, ``\textit{I like rules more because I know what's going into them. But with the prompts, you don't know what's going on. While the prompting is better at catching things, I just like the transparency of rules more}''.
Its transparency helps participants not only understand exactly why a comment was removed but also have more control over which specific comments should be removed. 
Although prompt filters allow people to write prompts that resemble rules, they might still remove comments with similar concepts. P8 compared the difference between rule filters and prompt filters along this dimension: ``\textit{[With the rule filter], you might get to really specific thing, and lost the big picture. But then [with the prompt filter], you have just these larger generalizations. You know you can't get down to the nitty-gritty and identify truly exactly what phrases you want to remove.}''



% P9: John Lee: It does, because I think there's like a fine line between filtering or or censoring. I think it's important to know why certain comments or text was filtered.

% The rules made it easy to cut out specific content while still leaving room for exceptions. The labeled examples were made it easy to rate comments, but wasn't always effective at detecting similar content. The prompts were straightforward to write, but got easily confused when I tried to filter content from a specific viewpoint


==> sections/deprecated.tex <==
Despite the indispensable role online communities (e.g. Facebook, Wikipedia, and YouTube) play in our daily lives, we still see with disappointment an overwhelming number of examples of spam, misinformation, and off-topic postings in our online experience. 
A nationally representative Pew Research Center study in 2017 found that roughly four in ten Americans had personally experienced online harassment \cite{PervasiveHarrassment}. 
Online platforms have adopted a variety of approaches to regulate online behavior and foster positive and productive conversations ~\cite{kiesler2012regulating}. 
Human moderators are employed by online platforms to regulate content \cite{roberts2016commercial, FacebookLabor} but face great challenges as the amount of content to be reviewed grows. 
Therefore, online communities like Facebook \cite{FacebookAlgorithm}, YouTube \cite{YoutubeAlgorithm}, and Reddit \cite{Chandrasekharan2019} increasingly adopt algorithms to automatically identify and remove damaging content at scale. 
However, centralized platform-wide moderation might fail to account for cultural variances across countries~\cite{jiang2021understanding}, communities~\cite{weld2022makes}, or diverse individual preferences, potentially leading to unintended harms. Besides, the lack of transparency of platform moderation processes has raised concerns among scholars and regulators regarding procedural fairness and accountability to the public~\cite{fan2020digital, suzor2018digital}. 

In today's social media, users often encounter content in their feeds not solely produced by individuals they follow. Besides, various platforms maintain different types of account-related information, ranging from reputation~\cite{movshovitz2013analysis}, the number of followers, to their history of being reported. In comparison, content-based tools focus directly on the content itself, making them more universally applicable across different platforms and scenarios. 
\subsubsection{Content Curation and Recommendation Systems}
Curation, in a social computing context, denotes the process of a curator selecting a subset of the
content that fits their preferences or the demand of a larger community, where the content can be
news articles, user submitted posts, or comments ~\cite{wang2022highlighting, feng2024mapping}.  For instance, editors at New York Times highlighted high-quality comments in their online comment sections. Many individual users also proactively curate for themselves through \textit{account-based} curation such as following or blocking certain users~\cite{lee2019consumptive}, or \textit{content-based} curation such as searching for specific tags or keywords~\cite{khatter2020analysis}. 

Content curation is also closely related to recommendation systems. While content curation often emphasizes the role of human in selecting, organizing, and sorting content, recommendation systems often rely on algorithms that that generate personalized feeds based on user interactions such as clicks, content dwell time~\cite{yi2014beyond}, and affinity with other users~\cite{kang2022you}). However, the growing research in \textit{integrative recommender systems} aims to integrate human values and preferences into recommendation systems, which gradually blurs the boundary between content curation and recommendation systems~\cite{he2023cura, burrell2019users, konstan2012recommender}. This approach often involves interactive features that allow users to provide direct input, such as toggles and sliders to adjust content characteristics, keyword critique~\cite{petrescu2021multi}, and thumb up/down buttons to rate recommended items~\cite{zhao2013interactive, yi2014beyond, kang2022you}. 

For instance, while advanced word filters have the potential to accommodating nuanced user preferences~\cite{song2023modsandbox}, it is often challenging and time-consuming for end-users to fully realize their potential~\cite{jhaver2019human}. People are frustrated at brainstorming various spelling variants and synonyms and at updating their filter to address false predictions. 
In general, content moderation and curation/recommendation systems are similar in that they both act on the
content one sees, where tuning a recommendation algorithm to reduce a specific type of content
may have a de facto effect akin to moderating it out.

Viewing personal moderation tools through a broader lens, we categorize them as a specific type of binary text filters and therefore draw inspiration from research in interactive machine learning. Essentially, end-users are engaged in teaching a binary algorithm to align with their unique preferences, all within the distinct context of personal moderation. In the following, we explore the challenges and needs end-users encounter when creating their personalized text filters, informing the research questions guiding our study. 

\begin{itemize}[leftmargin=0.5cm]
    \item \textbf{RQ3}: Which system can allow end users to build personalized text filters the most easily?
    \item \textbf{RQ3.1}: Which system can allow users to communicate their preferences to personalized text filters the most easily?
    \item \textbf{RQ3.2}: Which system can allow end users to iterate their personalized text filter the most easily?
\end{itemize}

Beyond its role in supporting iteration, explainability holds intrinsic value. 
Prior research has shown that exposing the reasoning and data behind the algorithmic decision can help improve users' acceptance of and satisfaction with the system~\cite{bostandjiev2012tasteweights, cramer2008effects}. 


Despite the growing enthusiasm for personal moderation tools, prior research has identified significant challenges associated with their use~\cite{jhaver2023personalizing, feng2024mapping}. 


\textbf{Effectiveness}. Existing personal moderation tools often fail to account for nuanced personal preferences, which might vary not only across individuals but also across the conversation context~\cite{jiang2021understanding, feng2024mapping}. For instance, marginalized communities might want to filter out derogatory terms used by outsiders but do not object to using them in internal group discussions. As a result, a generic filter designed to block racism or misogyny could inadvertently censor well-meaning conversations within these communities~\cite{jhaver2023personalizing}. 
Users also complained that static word filters often failed to adapt to the evolving nature of online slurs to remain effective~\cite{sood2012profanity}.  The challenge of creating effective personalized filters motivates the primary research question of our study:



\textbf{Efficiency}. Second, users also desire the ability to efficiently build their personalized text filters. Since many of them view social media as a leisure activity or a time-killer, configuring personal moderation settings is considered an additional burden to them~\cite{feng2024mapping, jhaver2022designing}. While they recognize the trade-offs between granular control and the labor required to finetune their personal classifier, they expect improvements to their social media feeds in proportion to the effort and time invested in setting up the corresponding configuration~\cite{jhaver2023personalizing}. Thus we also ask:

\textbf{Usability}. In addition to efficiency and effectiveness, usability emerges as a crucial criterion for personal moderation tools. There is often an inherent trade-off between usability and effectiveness. For instance, while people can easily remove unwanted content by category-based filters designed for common toxicity, these filters often fail to effectively align with their nuanced preferences. Prior research has also shown that humans are only willing to devote as much effort as is minimally satisfactory rather than aiming for optimal outcomes~\cite{simon1956rational, kool2010decision, buccinca2021trust}. 

Furthermore, we noted that the development of personal moderation filters is a continuous and iterative process. Users often engage in a cycle of training, feedback, and correction to bootstrap their text filters, a pattern typical in interactive machine learning ~\cite{fails2003interactive}. For instance, users often switch between adjusting filter settings and reviewing their content feeds to ensure their configurations meet their expectations~\cite{jhaver2023personalizing}. 
This iterative cycle does not conclude with the filter's initial configuration but continues over the long term.
Rather than creating a comprehensive text filter from the start, end-users might only identify their moderation needs upon encountering undesirable content.~\cite{jhaver2023personalizing}. In their everyday use of personal moderation filters, they also engage in continuous algorithmic auditing to identify harmful behaviors~\cite{shen2021everyday}. 
However, current personal moderation tools frequently lack the capability to let users dynamically iterate their moderation filters. While category-based filters remain static, end-users also complained about the challenges of creating complex rules to accommodate new patterns of unwanted content~\cite{song2023modsandbox}. Therefore, iterability is also a crucial factor when we evaluate the usability of personal moderation tools. 

With these challenges in mind, how should we design a better personal moderation system that carefully navigates these important design dimensions? 
While there is an increasing body of research developing personal moderation tools using a variety of techniques ~\cite{song2023modsandbox, Chandrasekharan2019, OpenAI2024GPT4}, little has actually compared the effectiveness of these techniques in fulfilling these design dimensions. Therefore, we would like to pause and conduct a comprehensive evaluation of these techniques. This will enable us to outline the direction for future systems in personal moderation.

However, AutoMod is designed for collaborative moderation within community settings and therefore not readily accessible to end-users interested in personal moderation. 
First, it requires users to write rules using the YAML scripting language. Users are expected to be not only familiar with the YAML syntax but also comfortable with scripting rather than a more intuitive user interface. 
Additionally, AutoMod's advanced pattern recognition features, such as regular expressions and diverse resultant actions, may be well-suited for Reddit's community moderators who are motivated to learn these technologies for community governance.
But these features can be overly complex for end-users seeking to leverage similar capabilities for their personal content moderation.
Given these challenges, we conducted several pilot studies to iteratively build a rule configuring system that is more user-friendly and suitable for end-users' moderation needs.

Each rule is defined by one or
more \textit{conditions} and resultant \textit{actions} (e.g., approval or removal). A condition examines whether a text includes a list of keywords, phrases, or regular expressions. The tool then verifies whether the field includes any listed keyword and phrase or matches any regular expression. Posts that satisfy all conditions of a rule will receive the designated action, such as removal or approval~\cite{reddit2023automod}.

% The most commonly used personal moderation tool is \textit{word filters}~\cite{jhaver2022designing}, where users can create a list of words to block, thereby filtering out or flagging content containing those words. Some platforms have introduced features enabling users to adjust their content sensitivity settings for various topics, such as racism, misogyny, and political views~\cite{Instagram2024, bhargava2019gobo, Bodyguard2024}. 

Despite these varying scenarios, they all involve end-users teaching a classifier to match their preferences. Through this lens, existing technical systems afford three primary teaching vocabularies. Users could \textit{label examples} to indicate their likes with recommendation algorithms, or \textit{author rules} that specify keywords to remove harmful content.

% Drawing inspiration from research in interactive machine learning (ML) and in-context learning, we implemented three representative personal moderation systems for experiments. Each system offers a unique approach to personal moderation and is recognized either for its popularity or potential in personal moderation. In the \textbf{\textsc{Label System}}, users train a ``black box'' ML algorithm by labeling examples. We further incorporate pretrained word-embeddings~\cite{devlin2018bert} and active learning~\cite{settles2009active} into the system to facilitate more accurate and rapid filter creation. In the \textbf{\textsc{Rule System}}, users train a decision tree by authoring rules. Although rules are widely used to express user preferences in many content moderation systems today, their granular nature can make it challenging for users to create effective rules~\cite{Chandrasekharan2019, song2023modsandbox}. Finally, reflecting the increased interest in leveraging large language models (LLMs) for content moderation~\cite{ma2023adapting, OpenAI2024GPT4}, users communicate with LLMs by writing prompts in the \textbf{\textsc{Prompt System}}. While LLMs have the potential to understand nuanced preferences, their effective use requires prompt engineering skills beyond many end-users' abilities. 

% To answer this question, we focus on personal content moderation as a case study. Personal content moderation refers to how end-users tailor their content feeds to their unique moderation preferences~\cite{jhaver2023personalizing, jhaver2023users, he2023cura, burrell2019users, konstan2012recommender}. 
% We choose personal content moderation as it illustrates three key user needs of creating a personalized binary filter. First, users desire the ability to build their personal moderation filters \textbf{quickly}. Since many view social media as a leisure activity or time-killer, users only want to spend limited time configuring personal moderation settings~\cite{feng2024mapping, jhaver2022designing}. Relatedly, \textbf{usability} is another crucial criterion for personal moderation filters. The creation process should be easy and less mentally demanding for end-users. In particular, we focus on two critical stages in the filter creation process: communicating preferences and iterating filters. Users first articulate their nuanced preferences in a format that filters can understand (e.g., compiling a list of relevant keywords for a word) and then identify and correct errors in the filter. Finally, the filters should \textbf{accurately} learn individual preferences, which can vary greatly in their complexity. There are great diversity and nuances in moderation preferences For example, while some users want to block common forms of racism or misogyny, marginalized communities might want to filter out derogatory terms used by outsiders but do not object to using them in internal group discussions~\cite{jhaver2023personalizing}.

% Looking forward, how might we design a better personal moderation system that carefully navigates these important design dimensions? 
% While there is an increasing body of research developing personal moderation tools using various techniques ~\cite{song2023modsandbox, Chandrasekharan2019, OpenAI2024GPT4}, few have \textit{compared} the effectiveness of these techniques in fulfilling these design dimensions. Therefore, we aim to first conduct a comprehensive evaluation of existing techniques to inform the direction for future personal moderation tools. 


% Corresponding to each strategy, we implemented a content curation system with state-of-the-art and comparable features for a fair comparison. In the \textbf{\textsc{Label System}}, users train a ``black box'' ML algorithm by labeling examples (Figure \ref{example labeling}). We further incorporate pretrained word-embeddings~\cite{devlin2018bert} and active learning~\cite{settles2009active} into the system to facilitate more accurate and rapid filter creation. In the \textbf{\textsc{Rule System}}, users train a decision tree by authoring rules. Users can
% interactively apply rules to examples of content to assess their rules’ effectiveness and adjust their rules accordingly. Finally, users communicate with LLMs by writing prompts in the \textbf{\textsc{Prompt System}}. 

% We discovered that the prompt system has a significantly higher recall in removing unwanted content compared to the other two systems, though it did not show higher precision in its removal predictions. Overall, it has a significantly higher $F_1$ score but only comparable accuracy to the other two systems. Further analysis of performance changes throughout the creation stage revealed a consistent trend: participants were able to create a filter that removed more unwanted content more efficiently with writing prompts. However, while participants were able to steadily remove more unwanted content with the prompt filter and the rule filter, they faced challenges in improving the precision of the removal decisions of these two filters. In addition, participants found these systems to be more mentally demanding and frustrating compared to the example system.


% We have completed three pilot experiments so far and have obtained some preliminary findings. We find that users can leverage prompts to develop filters with decent performance more efficiently compared to the other two systems. The example labeling system demonstrates fluctuating but generally increasing accuracy throughout the session. However, the final performances of the prompt writing system and the example labeling system are comparable. Second, we observe that rules and prompts excel in different aspects of user preference articulation. Rules are more adept at defining specific and clear-cut criteria, while prompts are more effective at capturing subtle sentiments or perspectives. Finally, we note that participants frequently engaged in debugging their prompts by adding falsely classified comments and adding more details to their prompt descriptions. However, due to the opaque nature of LLMs, participants struggled to pinpoint which aspects of their descriptions needed refinement. In contrast, they found the addition of incorrectly predicted comments to be a more intuitive method for improving their prompts.

% Our vision for the final system is still taking shape, but a few key features are emerging. First, it should consist of both rule and prompt blocks as users may find different instruction types beneficial for expressing various preferences. Second, users should start with writing prompts to convey their user preferences as our observations suggest that prompts efficiently establish a baseline for personal filters. Finally, we suggest using examples to help users clarify any ambiguities in their prompts. We should also employ rules to break down complex prompts into simpler, individual components, thereby providing more granular explanations for prompt predictions.

